Language Modeling Using Tensor Trains

We propose a novel tensor network language model based on the simplest tensor network (i.e., tensor trains), called `Tensor Train Language Model' (TTLM). TTLM represents sentences in an exponential space constructed by the tensor product of words, but computing the probabilities of sentences in a low-dimensional fashion. We demonstrate that the architectures of Second-order RNNs, Recurrent Arithmetic Circuits (RACs), and Multiplicative Integration RNNs are, essentially, special cases of TTLM. Experimental evaluations on real language modeling tasks show that the proposed variants of TTLM (i.e., TTLM-Large and TTLM-Tiny) outperform the vanilla Recurrent Neural Networks (RNNs) with low-scale of hidden units. (The code is available at https://github.com/shuishen112/tensortrainlm.)

==> sections/backgrounds.tex <==
\section{Preliminaries}
\label{sec:tensor}

% % The uncertainty is one of the key foundations in the QT. The \emph{superposition} implies the uncertainty for a single particle while uncertainty for an ensemble system with multiple particles is described in a mixed system with measurement operations.

% \subsubsection{Superposition}
%  Algebraically, a particle in microscope world (e.g. atoms or photons) is described by vectors a multi-dimensional space. In a 2-dimensional case, in which two basis vectors are named as $\ket{0}$ and $\ket{1}$, \emph{Superposition} can be implemented as a linear combination of the basis vectors with complex-valued weights.  
% \begin{equation}   
% \ket{\phi} = \alpha_0 \ket{0} + \alpha_1 \ket{1}, 
% \end{equation} 
% where $0 \leq |\alpha_0|^2 \leq 1 $, $0 \leq |\alpha_1|^2 \leq 1 $  and $ |\alpha_0|^2 + |\alpha_1|^2 = 1$.  $\alpha$'s are complex scalars and $\ket{0}$ and $\ket{1}$ are vectors in complex vector space.   
% %The state $\ket{\phi}$ is said to be a superposition of the states $\ket{0}$ and $\ket{1}$, and the scalars $\alpha_0$ and $\alpha_1$ denote the amplitudes of the superposition. 
% %When either $|\alpha_0|^2$ or $|\alpha_1|^2$ is $1$, the particle corresponds to a classical bit; when $|\alpha_0|^2 = 1$, then $|\alpha_1|^2 = 0$ and $\ket{\phi} = \ket{0}$, and vice versa. It can be shown that the general particle state vector is normalized. 

% \subsubsection{Mixed system and Measurements}
% An ensemble system with multiple particles is called a \emph{mixed system}, in which the probability distribution is encapsulated by  a  positive semi-definite with unitary trace i.e. density matrix  
% \begin{equation} 
% \rho = \alpha_i \ket{\phi_i} \bra{\phi_i} 
% \end{equation} 
% In order to infer the possible state of this mixed system, Gleason's theorem \cite{gleason1957measures,hughes1992structure} is used  to calculate probability in quantum physics through measurements $\ket{M}$, i.e.
% \begin{equation} 
% \label{trace_measurement}
% P_M(\rho) =  \bra{M} \rho \ket{M} =tr(\rho \ket{M} \bra{M} ) 
% \end{equation}
% Although the off-diagonal elements pf $\rho$ is complex-valued, the $P_M(\rho)$  is guaranteed to be real-valued, since both  $\rho$ and $\ket{M} \bra{M}$ are Hermitian.

% \subsection{Semantic Hilbert Space}
% \label{semantic_hilbert_space}
% Here we introduce the Semantic Hilbert Space $\mathcal{H}$ defined on a complex vector space $\mathcal{C}^n$, and three different linguistic units, namely sememes, words and word combinations on the space. The concept of semantic measurement is introduced at last.

% % For convenience purposes, we follow the Dirac notations, which are widely used in quantum probability. Basically, a unit vector $\vec{\mu}$ and its transpose $\vec{\mu}^T$ are denoted as a ket $\vert u \rangle$ and a bra $\langle u \vert$ respectively. 

% % \subsubsection{Sememe}

% \textbf{Sememes.} 
% We assume $\mathcal{H}$ is spanned by the set of orthogonal basis states $\{\ket{e_j}\}_{i=1}^n$ for \textit{sememes}, which are the minimum semantic units of word meanings in language universals~\cite{goddard1994semantic}. Semantic units with larger granularities are based on the set of sememe basis.

% % \subsubsection{Word}
% % \label{sec:word}
% \textbf{Words.} 
% Words are  composed of sememes in superposition. Each word $w$ is a superposition over all sememes $\{\ket{e_j}\}_{i=1}^n$, or equivalently a unit-length vector on $\mathcal{H}$:
% \begin{equation}
% \label{superposition}
% \vert w \rangle =  \sum_{j=1}^n r_j e^{i\phi_j} \vert e_j \rangle
% \end{equation}
% In the expression above, $\{r_j\}_{j=1}^n$ are non-negative real-valued amplitudes satisfying $\sum_{j=1}^n {r_j}^2$ =1 and $\phi_j \in [-\pi,\pi]$ are the corresponding complex phases. 

% % We could also transfer the complex number in a complex plane as $re^{i\phi} = \cos\phi + i\sin\phi $.

% % We assume there are $n$ semantic concepts $\{C_i\}_{i=1}^{n}$ in the text collection, which could be considered as a limited The Hilbert Space $\mathcal{H}$ is then an n-dimensional finite space, where the concepts form a set of pure orthonormal states of the space, denoted as $\{\vert e_i \rangle\}_{i=1}^n$. 

% % \subsubsection{Semantic Composition}
% % \label{sentence_rep}
% \textbf{Semantic Composition.} 
% We view a combination of words (e.g. phrase, $n$-gram, sentence or document) as a mixed system composed of individual words, and its representation is computed as follows:
% \begin{equation}
% \label{mixture_old}
% \rho = \sum^m_j { \frac{1}{m} \ket{w_j} \bra{w_j}},
% \end{equation}
% where $m$ is the number of words and $\ket{w_j}$ is word superposition state in Eq.~\ref{superposition}, allowing multiple occurrences. Eq.~\label{mixture_old} produces a density matrix $\rho$ for semantic composition between words.
% %It describes a non-classical distribution over the set of sememes:  the complex-valued off--diagonal elements describes the correlations between sememes, while the diagonal entries (guaranteed to be real by its original property) correspond to a standard probability distribution. The off--diagonal elements provide our framework some potentials to model the possible interactions between the basic sememe basis, which was usually considered mutually independent with each other.

% %, which may give rise to emerging meanings when words are combined. 

% % \subsubsection{Semantic Measurement}
% \textbf{Semantic Measurement.} 
% The high-level features of a sequence of words are extracted through
% measurements on its mixed state. Given a density matrix $\rho$ of a mixed state, a rank-one projector $P$, which is the outer product of a unit complex vector, i.e. $P_{M_i}=\ket{M_i}\bra{M_i}$, is applied as a measurement projector. It is worth mentioning that $\ket{M_i}$ could be any state in this Hilbert space (not only limited to a specific word $w$).
% The measured probability is computed by Gleason`s Theorem ( Eq.~\ref{trace_measurement}), namely $P_{M_i}(\rho) =  \bra{M_i} \rho \ket{M_i} =tr(\rho \ket{M_i} \bra{M_i}$  . The measurement directions i.e. $\{\ket{M_i}\}_{i=0}^{n}$ are mutually orthogonal with each other, therefore we can get a normalized  multinomial probability distribution $\sum_{i=0}^{n}(P_{M_i}(\rho)) =1$.





% The advantages of the above Semantic Hilbert Space are threefold. First,  similarly to capsules \cite{sabour2017dynamic} and quaternions RNN \cite{parcollet2018quaternion}, Semantic Hilbert Space (SHS) can code internal dependencies by composing and processing multidimensional
% features as single entities, namely unitary states.
% Second, the measurements can be treated as general feature extractor based on some general pre-trained language model \cite{devlin2018bert}, which can provide some potential to transfer the learned measurements from a dataset to a new dataset. Finally, the words and measurements are embedded in a single Hilbert Space, making this framework easy to be understood by humans. Thus the model can be more robust and possible to be managed by manual adjustment.


\subsection{Tensors and the Tensor Product}

A \emph{tensor} is a natural way to describe certain objects that have a central role in modern quantum physics and beyond.  
% Compared to matrices and vectors, tensor is not very common-used in machine learning communities. However, tensors are everywhere and  it is getting more and more attentions.
A tensor is, roughly, a multi-dimensional array with certain composition properties. For example, A first-order tensor over the space
$\mathbb{R}^m$ is a vector ${\bf{v}} \in \mathbb{R}^{m}$ \footnote{In the rest of this paper, we also regard a matrix as a kind of tensor, namely  a 2-order tensor.}, and a second-order tensor is a matrix.  There are typical ways to build tensors through a set of matrices or vectors, namely \textit{stacking} and \textit{tensor product}.

\textbf{Stacking.} 
Stacking a series of $n$-order tensors could result in $n+1$-order tensors, namely, let $\tG_{1},\tG_{2} \cdots,\tG _{r_{n+1}} \in \mathbb{R}^{r_1 r_2 \cdots r_n}$,
\begin{equation}
[\tG_{1};\tG_{2} \cdots;\tG _{r_{n+1}} ] \in \mathbb{R}^{r_1 r_2 \cdots r_n r_{n+1}}
\end{equation}
In detail, the typical basic feature arrays  are  pixels of images in computer vision and  words of textual documents in natural language processing. It is commonly-used to stack the pixels with vertical and horizontal directions, resulting $\textrm{width} \times \textrm{height}$ 2-order matrices. Similarly, words, which are usually represented as distributed vectors, can be stacked as matrices while they are sequentially occurring in a document.
High-order arrays i.e. tensors are usually built by stacking with more than 2 dimensions. The extra orders \footnote{It is worthy mentioned that  data/features in a \textit{batch} can be stacked in deep learning approaches, resulting in a new order related to \textit{batch}; therefore, this is one of the reasons why Google named its deep learning framework as Tensorflow, that is a \textit{data flow with tensors}.} can be 1) \textbf{timestamp}: data which involves time, like google books and Arxiv paper collections; 2)  \textbf{modality}: data with multiple modality e.g. image, text and sound; 3) \textbf{domain}: data with multiple domains, like news in sport, economy and politics. 4)  \textbf{positional order}: data with a sequential order, for example, language;




\textbf{Tensor Product.} 
%The \textbf{order} of a tensor is defined to the number of indexing entries in the array, which are referred to as modes. The dimension of a tensor in particular mode is defined as the number of values that may be taken by the index in the mode. 
%A tensor $\mathcal{T} \in \mathbb{R}^{m_1 \times \ldots \times m_n}$ means that it is a $n$-order tensor with $m_i$ in each mode. 
\textit{Tensor product}, denoted by $ \otimes $, is typically as an operation on (pairs of) ordered set of objects, for example, sequential data like zig-zag pixels in images and tokens/words in text. Let $\tA \in \mathbb{R}^{m_{1}\times\cdots\times m_{I}}$ and $\tB \in \mathbb{R}^{m_{I+1}\times\cdots\times m_{J}}$ be tensors of orders $I$ and $J$, respectively. Then, $\tA \otimes \tB \in \mathbb{R}^{m_{1}\times\cdots\times m_{I+J}}$ is a tensor of order ${I+J}$.
The dimension of the tensor product between two tensors is  the product of the dimensions thereof, which is especially for sequential data like zig-zag pixels in images and tokens/words in text. 
The below is the example of the tensor product between two 2-order tensors (namely matrices):
\begin{equation}
\begin{aligned}
\begin{bmatrix}
 a_{1,1} & a_{1,2} \\
 a_{2,1} & a_{2,2} \\
 \end{bmatrix}
\otimes
 \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix}
&=
 \begin{bmatrix}
 a_{1,1} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} & a_{1,2} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} \\
 & \\
 a_{2,1} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} & a_{2,2} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} \\
 \end{bmatrix} \\
&=
 \begin{bmatrix}
  \begin{bmatrix}
 a_{1,1} b_{1,1} & a_{1,1} b_{1,2} & \\ a_{1,2} b_{1,1} & a_{1,2} b_{1,2} \\
  \end{bmatrix}
  \begin{bmatrix}
 a_{1,1} b_{2,1} & a_{1,1} b_{2,2} & \\ a_{1,2} b_{2,1} & a_{1,2} b_{2,2} \\
  \end{bmatrix} \\
  \begin{bmatrix}
 a_{2,1} b_{1,1} & a_{2,1} b_{1,2} & \\ a_{2,2} b_{1,1} & a_{2,2} b_{1,2} \\
  \end{bmatrix}
  \begin{bmatrix}
 a_{2,1} b_{2,1} & a_{2,1} b_{2,2} & \\ a_{2,2} b_{2,1} & a_{2,2} b_{2,2} \\
 \end{bmatrix}
 \end{bmatrix}.
\end{aligned}
\end{equation}
%We use
%<\cdot, \cdot>$ for the inner product between two tensors in same space, i.e., the sum of element-wise multiplication of two tensors.
% $\mathbb{R}^{m_{1}\times\cdots\times m_{I}}$
Let $\tT_{h_1,\cdots,h_n}  \in \mathbb{R}$ be a specific entry in a tensor. 
%$\tT$ will be referenced with subscripts, e.g. $\{h_1,\cdots,h_n\}$. 
The inner product of two same-sized tensors in $\mathbb{R}^{m_{1}\times\cdots\times m_{I}}$ is defined as 
\begin{equation}
    <\tA, \tB> = \sum_{ \{h^{(1)}, h^{(2)}, \cdots h^{(n)}\} \in \mathbb{I}} \mathcal{\tA}_{h_1,\cdots,h_n} \mathcal{\tB}_{h_1,\cdots,h_n}
\end{equation}
where $\mathbb{I}$ is the index set of with dimension ${m_{1}\times\cdots\times m_{I}}$.

% A special $n$-order tensor $\delta \in \mathbb{R}^{k \times\ldots \times k }$, is as follows~\cite{2017arXiv170401552L,2015arXiv150905009C}:
% \begin{equation}
% \label{eq:function}
% {\delta _{{h_1}\ldots{h_n}}} = \left\{ \begin{array}{l}
% 1,\begin{array}{*{20}{c}}
% {}&{{h_1} = \dots = {h_n}}
% \end{array}\\
% 0,\begin{array}{*{20}{c}}
% {}&{otherwise}
% \end{array}
% \end{array} \right.
% \end{equation}
% with ${h_i} \in \left[ k \right]$. It means that it's $1$ for diagonal elements, $0$ for non-diagonal elements. It is mainly to construct the decomposition equivalent to Tensor Network (TN).


\subsection{Tensor  Decomposition}
\label{sec:ttd}

In practical applications, tensors usually involve operations on high-dimensional spaces, whence tensor decomposition is adopted to reduce the computing time. CP (CANDECOMP/Parafac) Decomposition and Tucker Decomposition (also called Multilinear SVD or M-mode SVD) are most typical ways.
CP decomposition fits the given tensor with a linear combination of some rank-1 tensors, whereas Tucker decomposition computes the orthonormal mode matrices of the tensor. However, the expressive power of  CP decomposition  is limited due to that it is a sum of only some rank-one tensors, and Tucker Decomposition has exponential in d number of parameters i.e., $\mathcal{O}(dnr+r^d)$, leading it to be only widely used for relatively-lower dimension especially three-dimensional tensor~ \cite{oseledets2011tensor}. 

For high-order tensors, Tensor Train Decomposition~ \cite{oseledets2011tensor} 
is an alternative way to approximate a high-order tensor with a collection of 3-order tensors~\footnote{The first and last tensors have order 2, but we can generally treat them as 3-order tensors with a extra dummy order of length one. }, which increases only linearly to the dimension (order) of the tensor.

For a given tensor $\tA \in \mathbb{R}^{m_1\times m_2 \times \cdots \times m_n}$, one wishes to find tensors $\mG_1, \tG_2, \ldots,\tG_{n-1} , \mG_n$ such that:
\begin{equation}
\begin{aligned}
&\mG_1 \in \mathbb{R}^{m_1 \times r_1} \\
&\tG_2 \in \mathbb{R}^{r_1 \times m_2 \times r_2}\\
&\vdots \\
&\tG_i \in \mathbb{R}^{r_{i-1} \times m_i \times r_i}\\
&\vdots \\
&\mG_n \in \mathbb{R}^{r_{n-1} \times m_n }
\end{aligned}
\end{equation}
such that
\begin{equation}
\label{eq:ttdecomposition}
\tA = \mG_1  \tG_2  ... \tG_{n-1}  \mG_n \in \mathbb{R}^{m_1\times m_2 \times \cdots \times m_n}
\end{equation}


where $*$ is the matrix multiplication operation and will be omitted in the following part of this paper. Observe that Eq.~\ref{eq:ttdecomposition} only involves the multiplications of 3-order tensors, resulting in efficient space and time cost \cite{oseledets2011tensor}. 




